Benchmarking LLMs on the Semantic Overlap Summarization Task

Semantic Overlap Summarization (SOS) is a constrained multi-document summarization task, where the constraint is to capture the common/overlapping information between two alternative narratives. In this work, we perform a benchmarking study of popular Large Language Models (LLMs) exclusively on the SOS task. Additionally, we introduce the PrivacyPolicyPairs (3P) dataset to expand the space of SOS benchmarks in terms of quantity and variety. This dataset provides 135 high-quality SOS data samples sourced from privacy policy documents. We then use a standard prompting taxonomy called TELeR to create and evaluate 905,216 distinct LLM-generated summaries over two SOS datasets from different domains, and we further conduct human evaluation on a subset of 540 samples. We conclude the paper by analyzing models' performances and the reliability of automatic evaluation. The code and datasets used to conduct this study are available at https://anonymous.4open.science/r/llm_eval-E16D.

==> fig/all_data_allsides.tex <==
\begin{table*}[!ht]\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccc}
\hline
Model                              & Dataset         & Level  & Sem-F1 & Sem-F1 & Sem-F1 & R-1 & R-2 & R-L & R-L- & BERTscore \\                       
&          &   & (USE) & (Distil) & (RoBERTa) &  &  &  & Sum & \\
\hline
lmsys/vicuna-13b-v1.5-16k          & all\_sides      & 0              & 0.25         & 0.3             & 0.3              & 0.16    & 0.07    & 0.12    & 0.13        & -0.29     \\
lmsys/vicuna-13b-v1.5-16k          & all\_sides      & 1              & 0.17         & 0.23            & 0.23             & 0.14    & 0.07    & 0.12    & 0.12        & -0.36     \\
lmsys/vicuna-13b-v1.5-16k          & all\_sides      & 2              & 0.18         & 0.24            & 0.23             & 0.15    & 0.07    & 0.12    & 0.13        & -0.33     \\
lmsys/vicuna-13b-v1.5-16k          & all\_sides      & 3              & 0.42         & 0.41            & 0.43             & 0.36    & 0.17    & 0.26    & 0.28        & 0.28      \\
lmsys/vicuna-13b-v1.5-16k          & all\_sides      & 4              & 0.47         & 0.45            & 0.48             & 0.37    & 0.19    & 0.28    & 0.29        & 0.3       \\
lmsys/vicuna-13b-v1.5              & all\_sides      & 0              & 0.24         & 0.29            & 0.28             & 0.17    & 0.08    & 0.13    & 0.14        & -0.29     \\
lmsys/vicuna-13b-v1.5              & all\_sides      & 1              & 0.2          & 0.26            & 0.25             & 0.16    & 0.08    & 0.13    & 0.13        & -0.3      \\
lmsys/vicuna-13b-v1.5              & all\_sides      & 2              & 0.42         & 0.41            & 0.42             & 0.36    & 0.17    & 0.26    & 0.28        & 0.28      \\
lmsys/vicuna-13b-v1.5              & all\_sides      & 3              & 0.42         & 0.41            & 0.43             & 0.35    & 0.16    & 0.26    & 0.27        & 0.27      \\
lmsys/vicuna-13b-v1.5              & all\_sides      & 4              & 0.45         & 0.43            & 0.45             & 0.37    & 0.18    & 0.27    & 0.29        & 0.28      \\
lmsys/vicuna-7b-v1.5-16k           & all\_sides      & 0              & 0.38         & 0.39            & 0.4              & 0.24    & 0.12    & 0.17    & 0.19        & -0.04     \\
lmsys/vicuna-7b-v1.5-16k           & all\_sides      & 1              & 0.5          & 0.49            & 0.5              & 0.34    & 0.17    & 0.26    & 0.26        & 0.24      \\
lmsys/vicuna-7b-v1.5-16k           & all\_sides      & 2              & 0.43         & 0.42            & 0.44             & 0.35    & 0.17    & 0.27    & 0.28        & 0.25      \\
lmsys/vicuna-7b-v1.5-16k           & all\_sides      & 3              & 0.38         & 0.38            & 0.39             & 0.34    & 0.16    & 0.25    & 0.27        & 0.26      \\
lmsys/vicuna-7b-v1.5-16k           & all\_sides      & 4              & 0.36         & 0.35            & 0.37             & 0.29    & 0.14    & 0.22    & 0.23        & 0.2       \\
lmsys/vicuna-7b-v1.5               & all\_sides      & 0              & 0.32         & 0.33            & 0.34             & 0.18    & 0.08    & 0.13    & 0.15        & -0.16     \\
lmsys/vicuna-7b-v1.5               & all\_sides      & 1              & 0.5          & 0.5             & 0.5              & 0.35    & 0.19    & 0.26    & 0.27        & 0.25      \\
lmsys/vicuna-7b-v1.5               & all\_sides      & 2              & 0.44         & 0.43            & 0.45             & 0.39    & 0.21    & 0.3     & 0.32        & 0.33      \\
lmsys/vicuna-7b-v1.5               & all\_sides      & 3              & 0.4          & 0.39            & 0.41             & 0.34    & 0.17    & 0.26    & 0.27        & 0.28      \\
lmsys/vicuna-7b-v1.5               & all\_sides      & 4              & 0.35         & 0.35            & 0.37             & 0.27    & 0.13    & 0.2     & 0.21        & 0.19      \\
meta-llama/Llama-2-13b-chat-hf     & all\_sides      & 0              & 0.58         & 0.57            & 0.59             & 0.26    & 0.13    & 0.17    & 0.2         & 0.21      \\
meta-llama/Llama-2-13b-chat-hf     & all\_sides      & 1              & 0.44         & 0.44            & 0.46             & 0.42    & 0.23    & 0.33    & 0.34        & 0.34      \\
meta-llama/Llama-2-13b-chat-hf     & all\_sides      & 2              & 0.54         & 0.49            & 0.52             & 0.35    & 0.16    & 0.25    & 0.26        & 0.29      \\
meta-llama/Llama-2-13b-chat-hf     & all\_sides      & 3              & 0.46         & 0.4             & 0.46             & 0.32    & 0.14    & 0.22    & 0.25        & 0.13      \\
meta-llama/Llama-2-13b-chat-hf     & all\_sides      & 4              & 0.5          & 0.46            & 0.51             & 0.32    & 0.14    & 0.22    & 0.24        & 0.2       \\
meta-llama/Llama-2-7b-chat-hf      & all\_sides      & 0              & 0.59         & 0.58            & 0.6              & 0.26    & 0.13    & 0.17    & 0.19        & 0.21      \\
meta-llama/Llama-2-7b-chat-hf      & all\_sides      & 1              & 0.6          & 0.57            & 0.59             & 0.42    & 0.23    & 0.32    & 0.32        & 0.38      \\
meta-llama/Llama-2-7b-chat-hf      & all\_sides      & 2              & 0.54         & 0.48            & 0.52             & 0.35    & 0.16    & 0.25    & 0.26        & 0.29      \\
meta-llama/Llama-2-7b-chat-hf      & all\_sides      & 3              & 0.5          & 0.45            & 0.49             & 0.33    & 0.14    & 0.24    & 0.24        & 0.26      \\
meta-llama/Llama-2-7b-chat-hf      & all\_sides      & 4              & 0.49         & 0.45            & 0.48             & 0.33    & 0.14    & 0.24    & 0.24        & 0.26      \\
mistralai/Mistral-7B-Instruct-v0.1 & all\_sides      & 0              & 0.53         & 0.52            & 0.54             & 0.32    & 0.13    & 0.21    & 0.21        & 0.25      \\
mistralai/Mistral-7B-Instruct-v0.1 & all\_sides      & 1              & 0.65         & 0.62            & 0.62             & 0.47    & 0.29    & 0.39    & 0.39        & 0.47      \\
mistralai/Mistral-7B-Instruct-v0.1 & all\_sides      & 2              & 0.53         & 0.47            & 0.52             & 0.36    & 0.17    & 0.26    & 0.26        & 0.29      \\
mistralai/Mistral-7B-Instruct-v0.1 & all\_sides      & 3              & 0.52         & 0.46            & 0.5              & 0.35    & 0.17    & 0.26    & 0.27        & 0.27      \\
mistralai/Mistral-7B-Instruct-v0.1 & all\_sides      & 4              & 0.52         & 0.47            & 0.51             & 0.37    & 0.18    & 0.27    & 0.27        & 0.29      \\
mistralai/Mistral-7B-Instruct-v0.2 & all\_sides      & 0              & 0.48         & 0.44            & 0.47             & 0.18    & 0.07    & 0.11    & 0.13        & 0.06      \\
mistralai/Mistral-7B-Instruct-v0.2 & all\_sides      & 1              & 0.64         & 0.64            & 0.63             & 0.45    & 0.25    & 0.36    & 0.36        & 0.45      \\
mistralai/Mistral-7B-Instruct-v0.2 & all\_sides      & 2              & 0.53         & 0.48            & 0.53             & 0.37    & 0.18    & 0.28    & 0.28        & 0.33      \\
mistralai/Mistral-7B-Instruct-v0.2 & all\_sides      & 3              & 0.52         & 0.48            & 0.54             & 0.38    & 0.19    & 0.29    & 0.29        & 0.32      \\
mistralai/Mistral-7B-Instruct-v0.2 & all\_sides      & 4              & 0.54         & 0.49            & 0.54             & 0.38    & 0.19    & 0.29    & 0.29        & 0.32      \\
mosaicml/mpt-7b-chat               & all\_sides      & 0              & 0.41         & 0.41            & 0.44             & 0.25    & 0.11    & 0.17    & 0.18        & 0.14      \\
mosaicml/mpt-7b-chat               & all\_sides      & 1              & 0.54         & 0.5             & 0.54             & 0.32    & 0.15    & 0.23    & 0.23        & 0.26      \\
mosaicml/mpt-7b-chat               & all\_sides      & 2              & 0.5          & 0.45            & 0.5              & 0.32    & 0.14    & 0.23    & 0.23        & 0.25      \\
mosaicml/mpt-7b-chat               & all\_sides      & 3              & 0.47         & 0.44            & 0.49             & 0.29    & 0.12    & 0.21    & 0.21        & 0.22      \\
mosaicml/mpt-7b-chat               & all\_sides      & 4              & 0.5          & 0.46            & 0.5              & 0.31    & 0.14    & 0.23    & 0.23        & 0.23      \\
mosaicml/mpt-7b-instruct           & all\_sides      & 0              & 0.59         & 0.57            & 0.6              & 0.28    & 0.2     & 0.23    & 0.24        & 0.25      \\
mosaicml/mpt-7b-instruct           & all\_sides      & 1              & 0.6          & 0.56            & 0.59             & 0.36    & 0.18    & 0.26    & 0.26        & 0.3       \\
mosaicml/mpt-7b-instruct           & all\_sides      & 2              & 0.52         & 0.46            & 0.5              & 0.28    & 0.12    & 0.2     & 0.2         & 0.18      \\
mosaicml/mpt-7b-instruct           & all\_sides      & 3              & 0.49         & 0.44            & 0.48             & 0.27    & 0.11    & 0.18    & 0.19        & 0.14      \\
mosaicml/mpt-7b-instruct           & all\_sides      & 4              & 0.53         & 0.5             & 0.53             & 0.28    & 0.15    & 0.2     & 0.22        & 0.17      \\
mosaicml/mpt-30b-chat              & all\_sides      & 0              & 0.57         & 0.56            & 0.58             & 0.27    & 0.14    & 0.18    & 0.19        & 0.2       \\
mosaicml/mpt-30b-chat              & all\_sides      & 1              & 0.52         & 0.51            & 0.54             & 0.25    & 0.14    & 0.19    & 0.2         & 0.17      \\
mosaicml/mpt-30b-chat              & all\_sides      & 2              & 0.46         & 0.44            & 0.47             & 0.22    & 0.09    & 0.15    & 0.16        & 0.11      \\
mosaicml/mpt-30b-chat              & all\_sides      & 3              & 0.44         & 0.42            & 0.47             & 0.2     & 0.08    & 0.14    & 0.15        & 0.07      \\
mosaicml/mpt-30b-chat              & all\_sides      & 4              & 0.45         & 0.44            & 0.48             & 0.23    & 0.1     & 0.16    & 0.16        & 0.09      \\
mosaicml/mpt-30b-instruct          & all\_sides      & 0              & 0.59         & 0.56            & 0.58             & 0.35    & 0.19    & 0.26    & 0.27        & 0.31      \\
mosaicml/mpt-30b-instruct          & all\_sides      & 1              & 0.6          & 0.56            & 0.57             & 0.39    & 0.19    & 0.32    & 0.32        & 0.41      \\
mosaicml/mpt-30b-instruct          & all\_sides      & 2              & 0.44         & 0.43            & 0.43             & 0.29    & 0.13    & 0.24    & 0.24        & 0.22      \\
mosaicml/mpt-30b-instruct          & all\_sides      & 3              & 0.48         & 0.47            & 0.47             & 0.33    & 0.14    & 0.28    & 0.27        & 0.27      \\
mosaicml/mpt-30b-instruct          & all\_sides      & 4              & 0.47         & 0.44            & 0.47             & 0.33    & 0.14    & 0.25    & 0.25        & 0.26      \\
chat-bison-001                     & all\_sides      & 0              & 0.55         & 0.52            & 0.54             & 0.22    & 0.09    & 0.15    & 0.17        & 0.15      \\
chat-bison-001                     & all\_sides      & 1              & 0.63         & 0.59            & 0.61             & 0.46    & 0.27    & 0.39    & 0.39        & 0.47      \\
chat-bison-001                     & all\_sides      & 2              & 0.5          & 0.46            & 0.49             & 0.35    & 0.16    & 0.26    & 0.26        & 0.28      \\
chat-bison-001                     & all\_sides      & 3              & 0.49         & 0.43            & 0.49             & 0.33    & 0.15    & 0.24    & 0.25        & 0.21      \\
chat-bison-001                     & all\_sides      & 4              & 0.55         & 0.5             & 0.54             & 0.37    & 0.18    & 0.28    & 0.28        & 0.3       \\
gpt-3.5-turbo                      & all\_sides      & 0              & 0.53         & 0.52            & 0.54             & 0.32    & 0.13    & 0.21    & 0.21        & 0.26      \\
gpt-3.5-turbo                      & all\_sides      & 1              & 0.63         & 0.59            & 0.62             & 0.48    & 0.28    & 0.41    & 0.41        & 0.46      \\
gpt-3.5-turbo                      & all\_sides      & 2              & 0.51         & 0.47            & 0.51             & 0.36    & 0.18    & 0.28    & 0.28        & 0.3       \\
gpt-3.5-turbo                      & all\_sides      & 3              & 0.51         & 0.47            & 0.51             & 0.37    & 0.18    & 0.27    & 0.28        & 0.28      \\
gpt-3.5-turbo                      & all\_sides      & 4              & 0.51         & 0.47            & 0.52             & 0.36    & 0.18    & 0.26    & 0.27        & 0.29      \\
gpt-4                              & all\_sides      & 0              & 0.6          & 0.57            & 0.6              & 0.37    & 0.17    & 0.25    & 0.25        & 0.32      \\
gpt-4                              & all\_sides      & 1              & 0.65         & 0.61            & 0.64             & 0.47    & 0.26    & 0.38    & 0.38        & 0.44      \\
gpt-4                              & all\_sides      & 2              & 0.58         & 0.51            & 0.56             & 0.41    & 0.2     & 0.29    & 0.29        & 0.33      \\
gpt-4                              & all\_sides      & 3              & 0.58         & 0.5             & 0.55             & 0.4     & 0.2     & 0.29    & 0.29        & 0.33      \\
gpt-4                              & all\_sides      & 4              & 0.6          & 0.53            & 0.58             & 0.4     & 0.2     & 0.3     & 0.3         & 0.35      \\
\hline
\end{tabular}%
}
\caption{All data collected on the AllSides dataset for our finalized set of prompts}
\label{tbl:alldataallsides}
\end{table*}

==> fig/all_data_privacypolicy.tex <==
\begin{table*}[!ht]\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccc}
\hline
Model                              & Dataset         & Level & Sem-F1 & Sem-F1 & Sem-F1 & R-1 & R-2 & R-L & R-L- & BERTscore \\                       
&          &   & (USE) & (Distil) & (RoBERTa) &  &  &  & Sum & \\
\hline
lmsys/vicuna-13b-v1.5-16k          & privacy\_policy & 0     & 0.17         & 0.26            & 0.27             & 0.06    & 0.02    & 0.05    & 0.05        & -0.38     \\
lmsys/vicuna-13b-v1.5-16k          & privacy\_policy & 1     & 0.15         & 0.24            & 0.23             & 0.1     & 0.03    & 0.08    & 0.08        & -0.32     \\
lmsys/vicuna-13b-v1.5-16k          & privacy\_policy & 2     & 0.25         & 0.37            & 0.41             & 0.19    & 0.05    & 0.14    & 0.15        & 0.1       \\
lmsys/vicuna-13b-v1.5-16k          & privacy\_policy & 3     & 0.23         & 0.34            & 0.36             & 0.14    & 0.04    & 0.1     & 0.1         & -0.12     \\
lmsys/vicuna-13b-v1.5-16k          & privacy\_policy & 4     & 0.29         & 0.4             & 0.44             & 0.18    & 0.05    & 0.13    & 0.14        & 0.08      \\
lmsys/vicuna-13b-v1.5              & privacy\_policy & 0     & 0.2          & 0.29            & 0.3              & 0.07    & 0.02    & 0.05    & 0.06        & -0.3      \\
lmsys/vicuna-13b-v1.5              & privacy\_policy & 1     & 0.19         & 0.29            & 0.29             & 0.11    & 0.04    & 0.09    & 0.09        & -0.22     \\
lmsys/vicuna-13b-v1.5              & privacy\_policy & 2     & 0.25         & 0.37            & 0.41             & 0.2     & 0.06    & 0.14    & 0.16        & 0.14      \\
lmsys/vicuna-13b-v1.5              & privacy\_policy & 3     & 0.25         & 0.38            & 0.41             & 0.17    & 0.05    & 0.12    & 0.13        & 0.08      \\
lmsys/vicuna-13b-v1.5              & privacy\_policy & 4     & 0.27         & 0.39            & 0.42             & 0.18    & 0.05    & 0.13    & 0.14        & 0.1       \\
lmsys/vicuna-7b-v1.5-16k           & privacy\_policy & 0     & 0.22         & 0.32            & 0.33             & 0.06    & 0.02    & 0.04    & 0.05        & -0.27     \\
lmsys/vicuna-7b-v1.5-16k           & privacy\_policy & 1     & 0.27         & 0.39            & 0.4              & 0.2     & 0.05    & 0.15    & 0.15        & 0.11      \\
lmsys/vicuna-7b-v1.5-16k           & privacy\_policy & 2     & 0.24         & 0.36            & 0.39             & 0.2     & 0.05    & 0.14    & 0.16        & 0.13      \\
lmsys/vicuna-7b-v1.5-16k           & privacy\_policy & 3     & 0.28         & 0.4             & 0.45             & 0.18    & 0.05    & 0.13    & 0.14        & 0.11      \\
lmsys/vicuna-7b-v1.5-16k           & privacy\_policy & 4     & 0.3          & 0.41            & 0.44             & 0.18    & 0.05    & 0.13    & 0.13        & 0.1       \\
lmsys/vicuna-7b-v1.5               & privacy\_policy & 0     & 0.21         & 0.31            & 0.31             & 0.06    & 0.02    & 0.04    & 0.05        & -0.26     \\
lmsys/vicuna-7b-v1.5               & privacy\_policy & 1     & 0.25         & 0.37            & 0.39             & 0.17    & 0.05    & 0.12    & 0.13        & 0.06      \\
lmsys/vicuna-7b-v1.5               & privacy\_policy & 2     & 0.24         & 0.36            & 0.39             & 0.2     & 0.05    & 0.14    & 0.16        & 0.13      \\
lmsys/vicuna-7b-v1.5               & privacy\_policy & 3     & 0.24         & 0.37            & 0.4              & 0.17    & 0.04    & 0.13    & 0.14        & 0.09      \\
lmsys/vicuna-7b-v1.5               & privacy\_policy & 4     & 0.24         & 0.37            & 0.4              & 0.18    & 0.05    & 0.13    & 0.14        & 0.1       \\
meta-llama/Llama-2-13b-chat-hf     & privacy\_policy & 0     & 0.29         & 0.4             & 0.44             & 0.1     & 0.03    & 0.07    & 0.09        & -0.07     \\
meta-llama/Llama-2-13b-chat-hf     & privacy\_policy & 1     & 0.29         & 0.38            & 0.41             & 0.23    & 0.07    & 0.17    & 0.18        & 0.16      \\
meta-llama/Llama-2-13b-chat-hf     & privacy\_policy & 2     & 0.3          & 0.41            & 0.46             & 0.18    & 0.05    & 0.13    & 0.14        & 0.11      \\
meta-llama/Llama-2-13b-chat-hf     & privacy\_policy & 3     & 0.29         & 0.41            & 0.45             & 0.18    & 0.04    & 0.13    & 0.13        & 0.1       \\
meta-llama/Llama-2-13b-chat-hf     & privacy\_policy & 4     & 0.28         & 0.39            & 0.43             & 0.16    & 0.04    & 0.11    & 0.12        & 0.07      \\
meta-llama/Llama-2-7b-chat-hf      & privacy\_policy & 0     & 0.29         & 0.39            & 0.43             & 0.09    & 0.03    & 0.06    & 0.07        & -0.08     \\
meta-llama/Llama-2-7b-chat-hf      & privacy\_policy & 1     & 0.32         & 0.44            & 0.46             & 0.23    & 0.07    & 0.17    & 0.17        & 0.16      \\
meta-llama/Llama-2-7b-chat-hf      & privacy\_policy & 2     & 0.31         & 0.42            & 0.46             & 0.19    & 0.04    & 0.13    & 0.14        & 0.11      \\
meta-llama/Llama-2-7b-chat-hf      & privacy\_policy & 3     & 0.31         & 0.41            & 0.46             & 0.18    & 0.04    & 0.13    & 0.13        & 0.11      \\
meta-llama/Llama-2-7b-chat-hf      & privacy\_policy & 4     & 0.3          & 0.42            & 0.44             & 0.18    & 0.05    & 0.14    & 0.14        & 0.11      \\
mistralai/Mistral-7B-Instruct-v0.1 & privacy\_policy & 0     & 0.3          & 0.4             & 0.45             & 0.14    & 0.04    & 0.1     & 0.1         & 0.02      \\
mistralai/Mistral-7B-Instruct-v0.1 & privacy\_policy & 1     & 0.28         & 0.4             & 0.41             & 0.22    & 0.06    & 0.17    & 0.17        & 0.17      \\
mistralai/Mistral-7B-Instruct-v0.1 & privacy\_policy & 2     & 0.31         & 0.42            & 0.46             & 0.2     & 0.05    & 0.14    & 0.14        & 0.12      \\
mistralai/Mistral-7B-Instruct-v0.1 & privacy\_policy & 3     & 0.3          & 0.42            & 0.45             & 0.19    & 0.05    & 0.14    & 0.14        & 0.12      \\
mistralai/Mistral-7B-Instruct-v0.1 & privacy\_policy & 4     & 0.31         & 0.42            & 0.46             & 0.2     & 0.05    & 0.14    & 0.14        & 0.12      \\
mistralai/Mistral-7B-Instruct-v0.2 & privacy\_policy & 0     & 0.24         & 0.37            & 0.4              & 0.05    & 0.01    & 0.03    & 0.04        & -0.17     \\
mistralai/Mistral-7B-Instruct-v0.2 & privacy\_policy & 1     & 0.33         & 0.45            & 0.48             & 0.24    & 0.09    & 0.19    & 0.19        & 0.21      \\
mistralai/Mistral-7B-Instruct-v0.2 & privacy\_policy & 2     & 0.31         & 0.41            & 0.47             & 0.21    & 0.05    & 0.15    & 0.15        & 0.15      \\
mistralai/Mistral-7B-Instruct-v0.2 & privacy\_policy & 3     & 0.31         & 0.42            & 0.47             & 0.21    & 0.05    & 0.14    & 0.15        & 0.14      \\
mistralai/Mistral-7B-Instruct-v0.2 & privacy\_policy & 4     & 0.31         & 0.43            & 0.47             & 0.21    & 0.06    & 0.15    & 0.15        & 0.15      \\
mosaicml/mpt-7b-chat               & privacy\_policy & 0     & 0.24         & 0.36            & 0.4              & 0.12    & 0.03    & 0.09    & 0.09        & -0.05     \\
mosaicml/mpt-7b-chat               & privacy\_policy & 1     & 0.27         & 0.39            & 0.41             & 0.19    & 0.04    & 0.14    & 0.14        & 0.09      \\
mosaicml/mpt-7b-chat               & privacy\_policy & 2     & 0.26         & 0.39            & 0.43             & 0.18    & 0.03    & 0.12    & 0.13        & 0.08      \\
mosaicml/mpt-7b-chat               & privacy\_policy & 3     & 0.27         & 0.39            & 0.42             & 0.17    & 0.04    & 0.12    & 0.13        & 0.08      \\
mosaicml/mpt-7b-chat               & privacy\_policy & 4     & 0.27         & 0.39            & 0.43             & 0.17    & 0.04    & 0.12    & 0.13        & 0.06      \\
mosaicml/mpt-7b-instruct           & privacy\_policy & 0     & 0.32         & 0.43            & 0.47             & 0.13    & 0.04    & 0.09    & 0.1         & -0.03     \\
mosaicml/mpt-7b-instruct           & privacy\_policy & 1     & 0.28         & 0.38            & 0.41             & 0.18    & 0.05    & 0.13    & 0.14        & 0.07      \\
mosaicml/mpt-7b-instruct           & privacy\_policy & 2     & 0.27         & 0.38            & 0.41             & 0.15    & 0.04    & 0.11    & 0.12        & 0.03      \\
mosaicml/mpt-7b-instruct           & privacy\_policy & 3     & 0.27         & 0.37            & 0.41             & 0.16    & 0.04    & 0.11    & 0.13        & 0.02      \\
mosaicml/mpt-7b-instruct           & privacy\_policy & 4     & 0.27         & 0.38            & 0.41             & 0.14    & 0.03    & 0.1     & 0.11        & 0         \\
mosaicml/mpt-30b-chat              & privacy\_policy & 0     & 0.29         & 0.41            & 0.45             & 0.12    & 0.04    & 0.08    & 0.09        & -0.01     \\
mosaicml/mpt-30b-chat              & privacy\_policy & 1     & 0.31         & 0.42            & 0.45             & 0.18    & 0.05    & 0.14    & 0.14        & 0.08      \\
mosaicml/mpt-30b-chat              & privacy\_policy & 2     & 0.31         & 0.41            & 0.45             & 0.11    & 0.03    & 0.08    & 0.09        & -0.02     \\
mosaicml/mpt-30b-chat              & privacy\_policy & 3     & 0.31         & 0.41            & 0.45             & 0.13    & 0.04    & 0.09    & 0.1         & 0         \\
mosaicml/mpt-30b-chat              & privacy\_policy & 4     & 0.31         & 0.42            & 0.45             & 0.14    & 0.04    & 0.11    & 0.11        & 0.02      \\
mosaicml/mpt-30b-instruct          & privacy\_policy & 0     & 0.27         & 0.38            & 0.42             & 0.15    & 0.05    & 0.11    & 0.12        & 0.03      \\
mosaicml/mpt-30b-instruct          & privacy\_policy & 1     & 0.28         & 0.38            & 0.4              & 0.22    & 0.06    & 0.18    & 0.18        & 0.21      \\
mosaicml/mpt-30b-instruct          & privacy\_policy & 2     & 0.29         & 0.4             & 0.44             & 0.19    & 0.05    & 0.14    & 0.14        & 0.11      \\
mosaicml/mpt-30b-instruct          & privacy\_policy & 3     & 0.28         & 0.4             & 0.44             & 0.19    & 0.05    & 0.14    & 0.15        & 0.11      \\
mosaicml/mpt-30b-instruct          & privacy\_policy & 4     & 0.28         & 0.39            & 0.41             & 0.18    & 0.04    & 0.14    & 0.14        & 0.08      \\
chat-bison-001                     & privacy\_policy & 0     & 0.26         & 0.36            & 0.4              & 0.09    & 0.02    & 0.07    & 0.08        & -0.1      \\
chat-bison-001                     & privacy\_policy & 1     & 0.33         & 0.44            & 0.47             & 0.26    & 0.1     & 0.21    & 0.22        & 0.23      \\
chat-bison-001                     & privacy\_policy & 2     & 0.32         & 0.42            & 0.47             & 0.22    & 0.06    & 0.16    & 0.16        & 0.15      \\
chat-bison-001                     & privacy\_policy & 3     & 0.33         & 0.44            & 0.48             & 0.2     & 0.06    & 0.15    & 0.16        & 0.14      \\
chat-bison-001                     & privacy\_policy & 4     & 0.33         & 0.44            & 0.48             & 0.22    & 0.07    & 0.17    & 0.17        & 0.16      \\
gpt-3.5-turbo                      & privacy\_policy & 0     & 0.34         & 0.44            & 0.48             & 0.14    & 0.05    & 0.1     & 0.11        & 0.04      \\
gpt-3.5-turbo                      & privacy\_policy & 1     & 0.34         & 0.46            & 0.49             & 0.27    & 0.1     & 0.22    & 0.22        & 0.26      \\
gpt-3.5-turbo                      & privacy\_policy & 2     & 0.33         & 0.44            & 0.49             & 0.21    & 0.06    & 0.15    & 0.15        & 0.15      \\
gpt-3.5-turbo                      & privacy\_policy & 3     & 0.34         & 0.44            & 0.49             & 0.22    & 0.07    & 0.16    & 0.16        & 0.16      \\
gpt-3.5-turbo                      & privacy\_policy & 4     & 0.34         & 0.45            & 0.49             & 0.23    & 0.07    & 0.16    & 0.16        & 0.17      \\
gpt-4                              & privacy\_policy & 0     & 0.31         & 0.42            & 0.47             & 0.13    & 0.04    & 0.09    & 0.1         & 0.01      \\
gpt-4                              & privacy\_policy & 1     & 0.34         & 0.47            & 0.49             & 0.26    & 0.08    & 0.2     & 0.2         & 0.22      \\
gpt-4                              & privacy\_policy & 2     & 0.33         & 0.45            & 0.5              & 0.22    & 0.06    & 0.15    & 0.15        & 0.17      \\
gpt-4                              & privacy\_policy & 3     & 0.33         & 0.45            & 0.5              & 0.21    & 0.05    & 0.14    & 0.14        & 0.15      \\
gpt-4                              & privacy\_policy & 4     & 0.34         & 0.46            & 0.5              & 0.22    & 0.06    & 0.15    & 0.15        & 0.17      \\
\hline
\end{tabular}%
}
\caption{All data collected on the PrivacyPolicy dataset using our finalized set of prompts}
\label{tbl:alldataprivacy}
\end{table*}


==> fig/annotation_instructions.tex <==
\begin{table*}[!htb]
\centering
\includegraphics[width=\linewidth]{resource/annotation_instructions.png}
\caption{A single sample from the 3P dataset. For each sample, you are given the category name, company names, the corresponding policy subsections, the count of words in each policy, and the $3$ reference summaries. The highlighted text shows the overlapping information.}
\label{fig:human_annotation}
\end{table*}

==> fig/annotator_agreement.tex <==
\begin{figure}[!htb]\vspace{-2mm}
    \centering
    \includegraphics[width=\linewidth]{resource/agreement}
    \vspace{-8mm}
    \caption{
        Pearson correlation and Kendall's $\tau$ scores between annotator scores and automatic evaluation metrics (higher is better).
        The ``comb'' subscript shows the combined score where the annotators sat with each other to settle on a final score for each annotation sample.
    }
    \label{fig:annotator_agreement}\vspace{-2mm}
\end{figure}

==> fig/avg_scores_per_lv.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[!htb]\small
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
\hline
\textbf{Dataset}   & {\textbf{Level}} & \textbf{BERT} & \textbf{R-1} & \textbf{R-2} & {\textbf{R-L}} & {\textbf{R-L-}} & {\textbf{Sem-F1}} & {\textbf{Sem-F1}} & {\textbf{Sem-F1}} \\

& & \textbf{score} &  & &  & {\textbf{Sum}} & {\textbf{(Distil)}} & {\textbf{(RoBERTa)}} & {\textbf{(USE)}} \\ \hline\hline

Privacy       & \multicolumn{1}{c|}{0}             & \multicolumn{1}{c|}{-0.069}            & 0.119                                 & \multicolumn{1}{c|}{0.035}           & \multicolumn{1}{c|}{0.085}           & \multicolumn{1}{c|}{0.095}               & \multicolumn{1}{c|}{0.398}                   & \multicolumn{1}{c|}{0.444}                    & \multicolumn{1}{c}{0.288}                \\
\multicolumn{1}{l|}{Policy}                          & \multicolumn{1}{c|}{1}             & \multicolumn{1}{c|}{0.139}             & \textbf{0.235}                        & \multicolumn{1}{c|}{\textbf{0.073}}  & \multicolumn{1}{c|}{\textbf{0.181}}  & \multicolumn{1}{c|}{\textbf{0.185}}      & \multicolumn{1}{c|}{0.438}                   & \multicolumn{1}{c|}{0.473}                    & \multicolumn{1}{c}{0.323}                \\
\multicolumn{1}{l|}{Pairs (3P)}                          & \multicolumn{1}{c|}{2}             & \multicolumn{1}{c|}{\textbf{0.160}}    & 0.223                                 & \multicolumn{1}{c|}{0.059}           & \multicolumn{1}{c|}{0.158}           & \multicolumn{1}{c|}{0.166}               & \multicolumn{1}{c|}{0.447}                   & \multicolumn{1}{c|}{0.501}                    & \multicolumn{1}{c}{0.330}                \\
\multicolumn{1}{l|}{}                          & \multicolumn{1}{c|}{3}             & \multicolumn{1}{c|}{0.135}             & 0.209                                 & \multicolumn{1}{c|}{0.053}           & \multicolumn{1}{c|}{0.149}           & \multicolumn{1}{c|}{0.155}               & \multicolumn{1}{c|}{0.452}                   & \multicolumn{1}{c|}{0.504}                    & \multicolumn{1}{c}{0.333}                \\
\multicolumn{1}{l|}{}                          & \multicolumn{1}{c|}{4}             & \multicolumn{1}{c|}{0.145}             & 0.214                                 & \multicolumn{1}{c|}{0.058}           & \multicolumn{1}{c|}{0.152}           & \multicolumn{1}{c|}{0.157}               & \multicolumn{1}{c|}{\textbf{0.462}}          & \multicolumn{1}{c|}{\textbf{0.511}}     & {\textbf{0.339}}  \\ \hline\hline


\multicolumn{1}{l|}{\multirow{5}{*}{AllSides}} & \multicolumn{1}{c|}{0}             & \multicolumn{1}{c|}{0.453}             & 0.460                                 & \multicolumn{1}{c|}{0.267}           & \multicolumn{1}{c|}{0.177}           & \multicolumn{1}{c|}{0.190}               & \multicolumn{1}{c|}{0.475}                   & \multicolumn{1}{c|}{0.493}                    & \multicolumn{1}{c}{0.481}                \\
\multicolumn{1}{l|}{}                          & \multicolumn{1}{c|}{1}             & \multicolumn{1}{c|}{\textbf{0.265}}    & \textbf{0.365}                        & \multicolumn{1}{c|}{\textbf{0.199}}  & \multicolumn{1}{c|}{\textbf{0.290}}  & \multicolumn{1}{c|}{\textbf{0.292}}      & \multicolumn{1}{c|}{\textbf{0.511}}          & \multicolumn{1}{c|}{\textbf{0.526}}           & \multicolumn{1}{c}{\textbf{0.525}}       \\
\multicolumn{1}{l|}{}                          & \multicolumn{1}{c|}{2}             & \multicolumn{1}{c|}{0.227}             & 0.327                                 & \multicolumn{1}{c|}{0.154}           & \multicolumn{1}{c|}{0.243}           & \multicolumn{1}{c|}{0.249}               & \multicolumn{1}{c|}{0.443}                   & \multicolumn{1}{c|}{0.473}                    & \multicolumn{1}{c}{0.475}                \\
\multicolumn{1}{l|}{}                          & \multicolumn{1}{c|}{3}             & \multicolumn{1}{c|}{0.239}             & 0.331                                 & \multicolumn{1}{c|}{0.152}           & \multicolumn{1}{c|}{0.243}           & \multicolumn{1}{c|}{0.252}               & \multicolumn{1}{c|}{0.437}                   & \multicolumn{1}{c|}{0.474}                    & \multicolumn{1}{c}{0.472}                \\
\multicolumn{1}{l|}{}                          & \multicolumn{1}{c|}{4}             & \multicolumn{1}{c|}{0.249}             & 0.332                                 & \multicolumn{1}{c|}{0.159}           & \multicolumn{1}{c|}{0.245}           & \multicolumn{1}{c|}{0.251}               & \multicolumn{1}{c|}{0.453}                   & \multicolumn{1}{c|}{0.489}                    & \multicolumn{1}{c}{0.486}                \\ \hline
%\hline\multicolumn{1}{l|}{AllSides* - 3P*}           & \multicolumn{1}{c|}{-}             & \multicolumn{1}{c|}{$0.105$}             & $0.130$                                 & \multicolumn{1}{c|}{$0.126$}           & \multicolumn{1}{c|}{$0.109$}           & \multicolumn{1}{c|}{$0.107$}               & \multicolumn{1}{c|}{$0.049$}                   & \multicolumn{1}{c|}{$0.015$}                    & \multicolumn{1}{c}{$0.186$}                \\ \hline
\end{tabular}
}
    \caption{
        Average scores per metric broken down by level and dataset. highest of each metric and dataset are in bold. 
        %The bottom row shows the difference between the best scores on the AllSides data and the 3P data along each column.
    }
    \label{tbl:avg_scores_per_lv}
\end{table*}


==> fig/max_scores_per_model.tex <==
\begin{figure*}[t!]
    \includegraphics[width=\linewidth]{resource/max_scores_per_model.png}
    \caption{
        Best scores over each TeLER prompt level for all $16$ evaluated LLMs and for each dataset. Red shows BERTscore, green shows ROUGE, and blue shows Sem-F1. 
    }
    \label{fig:maxscorespermodel}
\end{figure*}

==> fig/max_scores_per_model_family.tex <==
\begin{figure*}[!htb]
    \centering
    \includegraphics[width=1\linewidth]{resource/max_scores_per_model_family.png}
    \vspace{-3mm}
    \caption{
        Best scores over each TeLER prompt level for the largest model of each family of LLMs and for each dataset. Red shows BERTscore, green shows ROUGE, and blue shows Sem-F1. A full breakdown of max scores obtained by each model is shown in Appendix \ref{appendix:figures}
        %\santu{mention that 13 models can be found in the appendix.}
    }
    \label{fig:maxscorespermodelfamily}\vspace{-2mm}
\end{figure*}
%\santu{axis labels need to increase in font size, so do the legends. Pull the legends outside the bar area.}


==> fig/prompt_group_trials.tex <==
\begin{table}[!htb]
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lccccc}
        \hline
        Prompt Group     & A             & B             & C    & D    & E    \\
        \hline\hline
        Sem-F1 (USE)     & \textbf{0.37} & 0.35          & 0.34 & 0.34 & 0.34 \\
        Sem-F1 (Distil)  & \textbf{0.41} & 0.40          & 0.39 & 0.39 & 0.39 \\
        Sem-F1 (RoBERTa) & \textbf{0.44} & 0.43          & 0.41 & 0.42 & 0.41 \\
        Rouge-1          & \textbf{0.24} & 0.23          & 0.22 & 0.22 & 0.22 \\
        Rouge-2          & \textbf{0.10} & 0.09          & 0.08 & 0.09 & 0.09 \\
        Rouge-L          & \textbf{0.17} & \textbf{0.17} & 0.16 & 0.16 & 0.16 \\
        Rouge-L Sum      & \textbf{0.18} & 0.17          & 0.16 & 0.17 & 0.17 \\
        BERTscore        & \textbf{0.11} & 0.09          & 0.05 & 0.07 & 0.06 \\
        \hline
    \end{tabular}%
    }
    \caption{
        Average evaluation scores for each prompt trial. 
        Each of these trials are made up from $1$ of each level of TeLER prompt from levels $0$ to $4$
    }
    \label{tbl:prompt_group_trials}
\end{table}

==> fig/response_lengths.tex <==
% \begin{table}[!htb]\small
% \centering
% \begin{tabular}{r|c|c}\hline
% \textbf{Template} & \textbf{\# Top Scores} & \textbf{Avg. Summ. Length} \\ \hline\hline
% ICL & 0 & 954.48 \\
% L0 & 7 & 1591.50 \\
% L1 & 140 & 871.76 \\
% L2 & 65 & 903.93 \\
% L3 & 36 & 598.84 \\
% L4 & 24 & 518.92 \\\hline
% \end{tabular}%

% \vspace{-3mm}
% \caption{
%     The average summary lengths compared to the number of top scores over each combination of model, metric, and prompt level.
%     These counts can be derived from Table \ref{tbl:best_scores}
% }
% \label{tbl:response_lengths}\vspace{-3mm}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering\small
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{l|cc|cc}\hline
 & \multicolumn{2}{c|}{AllSides} & \multicolumn{2}{c}{3P} \\ \cline{2-5}
\textbf{Template} & \begin{tabular}[c]{@{}c@{}}\textbf{\#} \textbf{Top} \\ \textbf{Scores}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Avg.} \\ \textbf{Summ.} \\ \textbf{Length}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\#} \textbf{Top} \\ \textbf{Scores}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Avg.} \\ \textbf{Summ.} \\ \textbf{Length}\end{tabular} \\ \hline\hline
ICL & 2 & 936.09 & 5 & 973.14 \\
L0 & 2 & 1337.85 & 2 & 1848.9 \\
L1 & 106 & 840.66 & 122 & 903.32 \\
L2 & 49 & 841.37 & 47 & 967.42 \\
L3 & 32 & 606.72 & 11 & 590.84 \\
L4 & 17 & 532.23 & 21 & 505.41\\\hline
\end{tabular}%
}
\caption{The average summary lengths compared to the number of top scores over each combination of model, metric, and prompt level.
(counts derived from Table~\ref{tbl:best_scores}).} \vspace{-4mm}
\label{tbl:response_lengths}
\end{table}

==> fig/score_distribution.tex <==
\begin{figure}[!htb]
    \includegraphics[width=\columnwidth]{resource/score_distribution.png}
    \vspace{-6mm}
    \caption{
        Distribution of scores from Sem-F1 (left) and final human annotator scores (right).
        %SEM-F1 scores range from 0 to 1 while annotator scores fall between 0 and 5.
    }
    \label{fig:score_distribution}\vspace{-2mm}
\end{figure}

==> fig/sos_for_privacy_policy.tex <==

\begin{figure*}[!htb]
	\centering
	\includegraphics[width=0.90\textwidth]{resource/Scenario.png}
        \vspace{-2mm}
	\caption{Example of a SOS task using two alternative privacy policy narratives.}
	 \label{fig:sos_for_privacy_policy}
  \vspace{-3mm}
\end{figure*}
%\santu{describe this figure in the intro as a motivating example of the SOS task.}

==> fig/teler_l0_templates.tex <==
\begin{figure}
\begin{lstlisting}
common:
  - "{{doc1}} {{doc2}}"
\end{lstlisting}
\caption{The contents of the templates for TELeR L0}
\label{lst:teler_l0_templates}
\end{figure}

==> fig/teler_l1_templates.tex <==
\begin{figure*}\tiny
\begin{lstlisting}
common:
  - |
    Document 1:
    {{doc1}}


    Document 2:
    {{doc2}}


    In one sentence, please tell me the overlapping information between Document 1 and Document 2

  - |
    Document 1:
    {{doc1}}


    Document 2:
    {{doc2}}


    summarize the overlapping information between the documents.

  - |
    Document 1:
    {{doc1}}


    Document 2:
    {{doc2}}


    output the overlapping information between the documents.

  - |
    Document 1:
    {{doc1}}


    Document 2:
    {{doc2}}


    output the common information between the documents.

  - |
    Document 1:
    {{doc1}}


    Document 2:
    {{doc2}}


    output only the overlapping information

all_sides:
  - |
    Document 1:
    {{doc1}}


    Document 2:
    {{doc2}}


    In one sentence, please tell me the overlapping information between article 1 and article 2

  - |
    Document 1:
    {{doc1}}


    Document 2:
    {{doc2}}


    summarize the overlapping information between the articles

  - |
    Document 1:
    {{doc1}}


    Document 2:
    {{doc2}}


    output the overlapping information of the events covered in these articles


privacy_policy:
  - |
    Policy 1:
    {{doc1}}


    Policy 2:
    {{doc2}}


    In one sentence, please tell me the overlapping information between policy 1 and policy 2

  - |
    Policy 1:
    {{doc1}}


    Policy 2:
    {{doc2}}


    summarize the information that the two policies share

  - |
    Policy 1:
    {{doc1}}


    Policy 2:
    {{doc2}}


    what is the shared information between the two policies
\end{lstlisting}
\caption{The contents of the templates for TELeR L1}
\label{lst:teler_l1_templates}
\end{figure*}

==> fig/top_prompts.tex <==
\begin{figure}[!htb]
    \includegraphics[width=0.9\linewidth]{resource/top_prompts_by_lv.png}
    \caption{
        Percentage of top prompts by level for each combination of model and metric (out of 240 variations). 
        Level 1 prompts generally outperform the other TeLER levels for these datasets. 
        The number $240$ comes from the different combinations of LLMs ($15$), metrics ($8$), and datasets ($2$), giving us $\text{\# LLMs} \times \text{\# Metrics} \times \text{\# Datasets} = 15\times 8\times 2 = 240$
    }
    \label{fig:top_prompts}
\end{figure}

==> section/unused/background_REMOVED.tex <==

\section{Background}

\subsection{Semantic Overlap Summarization Task}

Semantic Overlap Summarization (SOS) is a task aimed at extracting and condensing shared information between two input documents, $D_A$ and $D_B$. The output, denoted as $D_O$, is generated in natural language and only includes information present in both input documents. 
The task is framed as a constrained multi-seq-to-seq (text generation) task, where brevity is emphasized to minimize the repetition of overlapping content. The output can be extractive summaries, abstractive summaries, or a combination of both~\cite{sofsat}.

% SOS draws inspiration from set-like intersection operations, envisioning the shared information between documents as the intersection of sets \cite{sofsat}. 
% The aim is to provide an abstract summary of the overlapping information, disregarding redundant repetitions. 
Furthermore, SOS adheres to the commutative property, meaning the order of input documents doesn't affect the output summary; $D_A \cap_{O} D_B = D_B \cap_{O} D_A$. 
To facilitate research in this area, \citet{semantic_overlap} introduced the AllSides dataset for training and evaluation, which we also used for evaluation in this work.


%In this study we evaluate on two datasets for the SOS task: the AllSides dataset which was previously presented by \cite{semantic_overlap} and our newly introduced \textit{PrivacyPolicyPairs} (3P) dataset.

% With the introduction of the SOS task, the applicability of existing evaluation metrics came into question. 
% In their research, \citet{semf1} found ROUGE \cite{rouge} to have low correlation with human evaluations and introduced a new metric called Sem-F1. Sem-F1 is an automatic summary evaluation algorithm that utilizes sentence-level embeddings from models like USE \cite{use} and RoBERTa \cite{roberta} to compute sentence-wise semantic similarity.
% This new metric showed higher correlation with human judgements compared to ROUGE, making it the preferred method for evaluating SOS summaries.



\subsection{Prompting With TELeR Taxonomy}\label{sec:teler}

%\santu{Show the figure of the taxonomy from the original paper here and describe the taxonomy briefly.}



As shown in Figure~\ref{TELeR_Fig}, the TELeR taxonomy introduced by \citet{teler} categorizes complex task prompts based on four criteria. 

\begin{enumerate}[leftmargin=*,itemsep=0.2ex,partopsep=-0.8ex,parsep=-0.2ex]
    
    \item \textbf{Turn}: This refers to the number of turns or shots used while prompting an LLM to accomplish a complex task. In general, prompts can be classified as either single or multi-turn.
    
    \item \textbf{Expression}: This refers to the style of expression for interacting with the LLM, such as questioning or instructing. 
    
    %\item \textbf{Level of Details}: This dimension of prompt style deals with the granularity or depth of question or instruction. Prompts with higher levels of detail provide more granular instructions. For example, Level 0 has no directive, \ie, questions or instructions. On the other hand, Level 4 prompts have to specify the particular sub-tasks, an explanation of the output, and the basis for evaluation of the output generated by the LLM.
    \item \textbf{Level of Details}: This dimension of prompt style deals with the granularity or depth of question or instruction. Prompts with higher levels of detail provide more granular instructions. %For example, level 0 has no directive, \ie, questions or instructions, whereas level 1 prompts do. 
    
    \item \textbf{Role}: LLMs can provide users with the option of specifying the role of the system. The response of LLM can vary due to changes in role definitions in spite of the fact that the prompt content remains unchanged.
\end{enumerate}

The taxonomy outlines $7$ distinct levels starting from level 0 to level 6.
With each increase in level comes an increase in complexity of the prompt.
In level 0, only data/context is provided with no further instruction.
Level 1 extends level 0 by providing single-sentence instruction.
Then level 2 extends level 1, and so on, until level 6, where all characteristics of previous levels are provided along with the additional instruction for the LLM to explain its output. For more details on the TELeR taxonomy and its applications, see~\citet{teler}.
For convenience, we include the outline diagram from the paper in Appendix \ref{appendix:prompt_design}.


%\santu{You need to write a related work section here and connect this work to existing literature.}

==> section/unused/discussions_COMBINED_WITH_RESULTS.tex <==

\section{Discussion}
%\santu{You need to have a discussion section where you summarize your findings and present them in an easily digestible fashion.}
The main takeaways from our study are as follows:

\vspace{-2mm}
\begin{boxI}\small
\textit{\textbf{Finding-1}:  ``3P'' dataset is harder than ``AllSides'' for LLMs in the context of SOS task.}
\end{boxI}

To elaborate, Table~\ref{tbl:avg_scores_per_lv} shows a clear difference in scores between the AllSides data and the 3P data. 
These differences can possibly be explained for the following reasons.
The average document word count for both datasets has a significant difference but is well within the context windows of LLMs.
For the AllSides data, the average is $504.51$ while for the 3P data, it's $662.01$.
Another difference worth noting is the amount of overlapping tokens present in each dataset.
Utilizing the NLTK library \citep{nltk} for tokenization, we find that the AllSides dataset has an average of 23.36\% unique token overlap between source documents while it's 17.95\% only for 3P.
Aside from the numerical differences, it is also important to note the compositional differences between these datasets. The AllSides data is comprised of news articles that cover the same events.
By the nature of covering the same events, it is more likely for overlapping spans of text to occur in the form of quotes or headlines.
In contrast, although the documents of the 3P dataset are similar in terms of their document structure and the types of excerpts they fall under, but they are not essentially written about the same subjects. Each document pair in the 3P dataset represents two different companies whose policies can differ greatly while using similar language.

%the difference may arise due to the abundance of news data in the pertaining corpus in comparison to privacy policy data, which is of limited quantity compared to the real world event narratives. 
%Interestingly, the average length of the generated summary for the AllSides data was $39.51$ words, while for the 3P data, it was $22.46$, indicating LLMs perhaps have seen more news data than privacy policy narratives.




% Certainly for ROUGE this would explain the difference in scores and could be explored for future work.


%While these lengths of text do not necessarily come near any of the models' max sequence limits, it is possible that the LLM response lengths scaled with the lengths of the source documents which could lead to worse scores .One explanation for this difference could be the differing sequence lengths. 

%These lengths do not come near any of the models' max sequence limits but it is possible that the LLM response lengths scaled with the lengths of the source documents which could lead to worse scores.
% This is because that while the average length of source document pairs for the 3P dataset are \textit{longer} than the AllSides data, the length of summaries for the 3P data are \textit{shorter}.
% The average count of words per summary in the AllSides data was $39.51$ words while for the 3P data it was $22.46$.
% Certainly for ROUGE this would explain the difference in scores and could be explored for future work.

\begin{boxI}\small
\textit{\textbf{Finding-2}: SEM-F1 remains the recommended evaluation metric for the SOS task.}
\end{boxI}

Figure \ref{fig:annotator_agreement} shoes that SEM-F1 has the best correlation with human annotators, while ROUGE continues to show its limitations which is consistent with previous findings~\cite{akter-etal-2022-revisiting}. 
SEM-F1 even shows measurable improvement over BERTscore which has become a very popular summarization metric to report.
However while SEM-F1 shows improvement over established metrics, it is still far too unreliable to trust over human annotators.
These correlation numbers are still too low to be considered trustworthy and highlight that further work needs to be done before we can put our faith in automatic summary evaluation numbers.
It is also important to note that like BERTscore, SEM-F1 also lacks interpretability since they both rely on encoder models to compute their scores.

\begin{boxI}\small
\textit{\textbf{Finding-3}: Use \textttt{gpt-3.5-turbo} with TELeR L2 prompts for best results in the SOS task}
\end{boxI}

As of the time of writing, closed-source commercial LLMs remain the top performers in text generation.
However he quality of open-source models are not too far off from \textttt{gpt-3.5-turbo} according to our human evaluators as noted in Table \ref{tbl:human_prefs} and most of our evaluated models even compete with \textttt{gemini-pro}.
Aside from model preferences it is also important to note that In-Context Learning styled prompts have been shown as a less effective prompting method compared to TELeR in the contstrained multi-document summarization setting.

% \begin{boxI}\small
% \textit{\textbf{Finding-2}: TELeR Level 1 generally outperforms other levels for the SOS task.}
% \end{boxI}

% This was a little puzzling to us as we expected more detailed/specific prompts would improve LLM's performance. But, looking retrospectively, this result may be explained by the fact the overlap summarizing task is still not very complex, and a single one-sentence instruction (Level 1) is sufficient for LLMs to understand the task properly.

% Therefore, we hypothesized that maybe the models struggled to follow complex directions (Levels 3 and 4) compared to the single-direction given at level $1$. However, upon further inspection of a few samples, we found it to not necessarily be the case.
% For example, with \texttt{gpt-3.5-turbo}, a sample with the level 1 prompt resulted in the following:

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.85\linewidth]{resource/l1_chat.png}
% \end{figure}

% However, in the case of the level 4 prompt, where explicit instructions are given to capture the common entities, events, and locations, we got:


% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.85\linewidth]{resource/l4_chat.png}
% \end{figure}


% Such an example could suggest limitations in the ability of the metrics to properly score responses with extra information such as \textit{"The common subjects are ..."} or a more common response such as \textit{"Sure, here is an example of ..."}.


%However in the case of the level 4 prompt where explicit instructions are given to capture the common subjects, events, and locations, we get the response:
%
%\begin{quote}
%"The common subjects between the two documents are Paul Manafort, his former business associate Rick Gates, and the charges they are facing. \\
%The common events between the documents are Manafort turning himself in at FBI headquarters and the unsealed indictment. \\
%The locations mentioned are Manafort's home in Alexandria, Virginia and the FBI field office in Washington D.C." \\
%\end{quote}

%Therefore, a more comprehensive study needs to be done, but 

%This shows that there are cases where the LLMs tend to address multiple points using multiple sentences whereas a single point can be addressed in a single sentence.
%A human annotator may rate the multi-sentence response highly but as noted in table \ref{tbl:ds_states}, our reference summaries fall between $1$ and $2$ sentences.




==> section/unused/related_REMOVED.tex <==


%\section{Related Work}
\subsection{Related Work}

% regular
% \cite{salience_alloc}

% multidoc
%  \cite{brio}
\textbf{Text Summarization:}  SOS is essentially a summarization task. Over the past two decades, many document summarization approaches have been investigated~\cite{zhong2019searching}. 
The two most popular among them are \textit{extractive} approaches \citep{cao-etal-2018-retrieve, narayan2018ranking, wu2018learning, zhong2020extractive} and \textit{abstractive} approaches \citep{bae2019summary, liu2017generative, nallapati2016abstractive}. 
Some researchers have tried combining extractive and abstractive approaches \citep{chen2018fast, hsu2018unified, zhang2019pegasus}. 

\smallskip
\noindent\textbf{Semantic Overlap Summarization:}
Semantic Overlap Summarization (SOS) is a task aimed at extracting and condensing shared information between two input documents, $D_A$ and $D_B$. 
The output, denoted as $D_O$, is generated in natural language and only includes information present in both input documents. 
The task is framed as a constrained multi-seq-to-seq (text generation) task, where brevity is emphasized to minimize the repetition of overlapping content. 
The output can be extractive summaries, abstractive summaries, or a combination of both~\cite{sofsat}.
This is similar to the sentence intersection task, where your input is comprised of sentences instead of documents and your output contains only the common information \citep{sent_intersect1,sent_intersect2}.

% SOS draws inspiration from set-like intersection operations, envisioning the shared information between documents as the intersection of sets \cite{sofsat}. 
% The aim is to provide an abstract summary of the overlapping information, disregarding redundant repetitions. 
Furthermore, SOS adheres to the commutative property, meaning the order of input documents doesn't affect the output summary; $D_A \cap_{O} D_B = D_B \cap_{O} D_A$. 
To facilitate research in this area, \citet{semantic_overlap} introduced the AllSides dataset for training and evaluation, which we also used for evaluation in this work.


%In this study we evaluate on two datasets for the SOS task: the AllSides dataset which was previously presented by \cite{semantic_overlap} and our newly introduced \textit{PrivacyPolicyPairs} (3P) dataset.

% With the introduction of the SOS task, the applicability of existing evaluation metrics came into question. 
% In their research, \citet{semf1} found ROUGE \cite{rouge} to have low correlation with human evaluations and introduced a new metric called Sem-F1. Sem-F1 is an automatic summary evaluation algorithm that utilizes sentence-level embeddings from models like USE \cite{use} and RoBERTa \cite{roberta} to compute sentence-wise semantic similarity.
% This new metric showed higher correlation with human judgements compared to ROUGE, making it the preferred method for evaluating SOS summaries.



% TODO: write another paragraph on multidocument summarization

%%%%% REDUNDANT INFO. SOS ALREADY COVERED IN BACKGROUND
% \smallskip
% \noindent\textbf{The SOS Task:} \textit{Semantic Overlap Summarization} can be framed as a multi-document summarization task, \ie multi-seq-to-seq task~\cite{goldstein2000multi,yasunaga2017graph, zhao2020summpip,ma2020multi,meena2014survey,lebanoff2018adapting,fabbri2019multi}. 
% However, unlike typical multi-document summarizing tasks, \textit{SOS} aims to summarize multiple alternative narratives with an overlapping constraint~\cite{semantic_overlap}, \ie the output should only contain the common information from both input narratives~\cite{karmaker2018sofsat}.
% The availability of data for this task is relatively small so recently \citet{sos_synthetic} proposed a method for training models by utilizing synthetically generated data.

% Transformers and LLMs Section
% \smallskip
% \noindent\textbf{Transformers and LLMs:} Encoder-decoder-based transformer models have recently gained a lot of attraction, especially for abstractive summarization tasks,~\cite{rush2015neural, chopra2016abstractive, zhou2017selective, paulus2017deep}. 
% Training a generic language model on a large corpus of data and then transferring/fine-tuning it for the summarization job has become a standard approach~\cite{radford2019better, devlin-etal-2019-bert, lewis2019bart, xiao2020ernie, yan2020prophetnet, zhang2019pegasus, raffel2019exploring}. Transformer architecture features more parallelizable training, better-scaling properties, and a built-in attention mechanism, allowing large language models (LLMs) to emerge. Made up of billions of parameters, many LLMs like GPT-2 \cite{gpt2}, and  LLaMA \cite{llama} have showcased strong abilities at generating text.
% Then, with the introduction of Reinforcement Learning From Human Feedback \cite{rlhf}, LLMs became even more powerful, allowing users to interact with them as data with natural language queries.



%In general, multiple document summarization is more challenging than single document summarization. 



% \smallskip
% \noindent\textbf{Transformers and LLMs:} For many years, the LSTM was the leading architecture for training neural language models \cite{lstm}.
% However in recent years, transformer architecture, introduced by \citet{attention_is_all_you_need}, has shown higher capabilities for sequence modeling tasks.

\smallskip\noindent\textbf{LLMs and Summarization:}
As the transformer architecture gained popularity, further research showed favorable behavior at scale, allowing the creation of larger and more performant models \citep{scaling1, scaling2, scaling3, scaling4, scaling5}.
With the rising prevalence of these large language models, summarization naturally became one of the many areas of NLP that have progressed as a result. 
Established tasks such as news summarization \citep{llm_news_sum} and multi-document summarization \citep{llm_multidoc_summ}




\smallskip\noindent\textbf{Prompt Engineering for LLMs:}  ``Prompt Engineering'' is a technique for maximizing the utility of LLMs in various tasks~\cite{zhou2022large}. It involves crafting and revising the query or context to elicit the desired response or behavior from LLMs~\cite{brown2022does}. Prompt engineering is an iterative process requiring multiple trial and error runs~\cite{shao2023compositional}. In fact, differences in prompts along several key factors can significantly impact the accuracy and performance of LLMs in complex tasks. To address this issue, \citet{teler} recently proposed the TELeR taxonomy, which can serve as a unified standard for benchmarking LLMs' performances by exploring a wide variety of prompts in a structured manner.


%\santu{Show the figure of the taxonomy from the original paper here and describe the taxonomy briefly.}



\label{sec:teler}
\smallskip\noindent\textbf{The TELeR Taxonomy:}
As shown in Figure~\ref{TELeR_Fig}, the TELeR taxonomy introduced by \citet{teler} categorizes complex task prompts based on four criteria. 

\begin{enumerate}[leftmargin=*,itemsep=0.2ex,partopsep=-0.8ex,parsep=-0.2ex]
    
    \item \textbf{Turn}: This refers to the number of turns or shots used while prompting an LLM to accomplish a complex task. In general, prompts can be classified as either single or multi-turn.
    
    \item \textbf{Expression}: This refers to the style of expression for interacting with the LLM, such as questioning or instructing. 
    
    %\item \textbf{Level of Details}: This dimension of prompt style deals with the granularity or depth of question or instruction. Prompts with higher levels of detail provide more granular instructions. For example, Level 0 has no directive, \ie, questions or instructions. On the other hand, Level 4 prompts have to specify the particular sub-tasks, an explanation of the output, and the basis for evaluation of the output generated by the LLM.
    \item \textbf{Level of Details}: This dimension of prompt style deals with the granularity or depth of question or instruction. Prompts with higher levels of detail provide more granular instructions. %For example, level 0 has no directive, \ie, questions or instructions, whereas level 1 prompts do. 
    
    \item \textbf{Role}: LLMs can provide users with the option of specifying the role of the system. The response of LLM can vary due to changes in role definitions in spite of the fact that the prompt content remains unchanged.
\end{enumerate}

The taxonomy outlines $7$ distinct levels starting from level 0 to level 6.
With each increase in level comes an increase in complexity of the prompt.
In level 0, only data/context is provided with no further instruction.
Level 1 extends level 0 by providing single-sentence instruction.
Then level 2 extends level 1, and so on, until level 6, where all characteristics of previous levels are provided along with the additional instruction for the LLM to explain its output. For more details on the TELeR taxonomy and its applications, see~\citet{teler}.
For convenience, we include the outline diagram from the paper in Appendix \ref{appendix:prompt_design}.


%\santu{You need to write a related work section here and connect this work to existing literature.}
